Hunting for the First Explosions at the High-Redshift Frontier

The James Webb Space Telescope (JWST) has spectroscopically confirmed galaxies up to $z\sim14$, 300 Myr after the Big Bang, and several candidates have been discovered at $z\sim15-25$, with one candidate as high as $z\sim30$, only 100 Myr after the Big Bang. Such objects are unexpected, since theoretical studies have not predicted the existence of detectable galaxies at $z\sim30$. While any $z\sim30$ candidates may be contaminants at lower redshifts, we explore whether such extreme redshift sources could be consistent with hyper-energetic transient events linked to the formation of the first, metal-free, stars. Specifically, we consider pair-instability supernovae (PISNe), a predicted class of extreme thermonuclear explosions that leave no remnant behind. Using cosmological simulations, we investigate an overdense cosmic region, where star formation and subsequent PISNe occur at $z\sim30-40$, even within standard cosmology. Assessing the likelihood of such a region, the corresponding number of PISNe at $z\gtrsim20$, and their observed flux, we find that JWST has a non-negligible chance to detect a PISN event at extremely high redshifts. If a transient event were confirmed at $z\sim30$, this would provide a direct glimpse into the epoch of first star formation, dramatically extending the empirical reach of astronomy.

==> abbrev.tex <==
% the list from ApJ
\newcommand{\aj}{AJ}
\newcommand{\apj}{ApJ}
\newcommand{\apjl}{ApJ}
\newcommand{\apjlett}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\apjsupp}{ApJS}
\newcommand{\aap}{A\&A}
\newcommand{\astap}{A\&A}
\newcommand{\araa}{ARA\&A}
\newcommand{\aapr}{A\&A Rev.}
\newcommand{\aaps}{A\&AS}
\newcommand{\mnras}{MNRAS}
\newcommand{\pasp}{PASP}
\newcommand{\apss}{Ap\&SS}
\newcommand{\pasj}{PASJ}
\newcommand{\nat}{Nature}
\newcommand{\sci}{Science}
\newcommand{\skytel}{S\&T}
\newcommand{\memras}{MmRAS}
\newcommand{\qjras}{QJRAS}
\newcommand{\jrasc}{JRASC}
\newcommand{\baas}{BAAS}
\newcommand{\iauc}{IAU Circ.}
\newcommand{\iaucirc}{IAU Circ.}
\newcommand{\aplett}{Astrophys. Lett.}
\newcommand{\apspr}{Astrophys. Space Phys. Res.}
\newcommand{\bain}{Bull. Astron. Inst. Netherlands}
\newcommand{\fcp}{Fund. Cosmic Phys.}
\newcommand{\aipconf}{AIP Conf. Proc.}
\newcommand{\aspconf}{ASP Conf. Ser.}
\newcommand{\asslconf}{Ap\&SSL Conf. Ser.}
\newcommand{\procspie}{Proc. SPIE}
\newcommand{\maps}{MAPS}
\newcommand{\planss}{Planet. Space Sci.}
\newcommand{\ssr}{Space Sci. Rev.}
\newcommand{\ao}{Appl. Opt.}
\newcommand{\applopt}{Appl. Opt.}
\newcommand{\solphys}{Sol. Phys.}
\newcommand{\pra}{Phys. Rev. A}
\newcommand{\prb}{Phys. Rev. B}
\newcommand{\prc}{Phys. Rev. C}
\newcommand{\prd}{Phys. Rev. D}
\newcommand{\pre}{Phys. Rev. E}
\newcommand{\prl}{Phys. Rev. Lett.}
\newcommand{\rmp}{Rev. Mod. Phys.}
\newcommand{\jcap}{J. Cosmology Astropart. Phys.}
% my additions

